Learning Enabled Fast Planning and Control in Dynamic Environments with Intermittent Information

This paper addresses a safe planning and control problem for mobile robots operating in communication- and sensor-limited dynamic environments. In this case the robots cannot sense the objects around them and must instead rely on intermittent, external information about the environment, as e.g., in underwater applications. The challenge in this case is that the robots must plan using only this stale data, while accounting for any noise in the data or uncertainty in the environment. To address this challenge we propose a compositional technique which leverages neural networks to quickly plan and control a robot through crowded and dynamic environments using only intermittent information. Specifically, our tool uses reachability analysis and potential fields to train a neural network that is capable of generating safe control actions. We demonstrate our technique both in simulation with an underwater vehicle crossing a crowded shipping channel and with real experiments with ground vehicles in communication- and sensor-limited environments.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Potential Fields}
Artificial potential fields are a well known method for path planning in robotics, particularly for navigating to a goal region while avoiding static obstacles. They work by defining an attractive field around the goal region and a repulsive field around each obstacle. See equations \ref{eqn:pfeqnAtt} and \ref{eqn:pfeqnRep}, respectively, for the exact field equations. 

\begin{align}
    U_{att}(q) = \frac{1}{2}K_p (\lvert \lvert q-q_{g}\rvert \rvert^2)
    \label{eqn:pfeqnAtt} \\
    U_{rep}(q) = \sum_i \frac{1}{2} K_r (\frac{1}{\lvert \lvert q-o_i \rvert \rvert})^2 \label{eqn:pfeqnRep}
\end{align}


These fields are then summed up, resulting in the composed field, shown in figure....

\begin{align}
    U= U_{att}(q) + U_{rep}(q) \label{eqn:composedField}
\end{align}

The motion planning algorithm then computes the next heading of the robot by following the negative gradient of the composed field. The gradient of the composed field is computed as follows.

\begin{align}
    \nabla U &= \nabla U_{att}(q) + \nabla U_{rep}(q)
\end{align}

\subsubsection{Properties}
Before moving on, we note some properties of potential fields which will be important later on. Potential fields are used because they are simple and fast to compute. They are also highly compositional, as the obstacle repulsive fields are simply summed up when computing the composed field. However, they are a reactive way of path planning, only considering the instantaneous state of the robot and the environment. They don't consider what may happen in the future. In addition, they can get stuck in local minima present in the composed field. Finally, dynamic environments also present the issue of dynamic minima. This mainly occurs when an obstacle repels the robot in the same direction that the obstacle is moving. See figure \ref{fig:dynamicMinima} for one such example of this phenomenon. We describe how to address these issues in section \ref{sec:approach}.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2375\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/image00000005.png}
        \caption{The robot approaches the obstacle, which is moving right} 
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2375\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{images/image00000009.png}
        \caption{The obstacle begins pushing the robot to the right}  
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.2375\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{images/image00000022.png}
        \caption{The obstacle pushes the robot in the same direction as the motion of the obstacle.}
        \label{fig:mean and std of net34}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2375\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{images/image00000039.png}
        \caption{The robot gets pushed by the obstacle, taking a much longer path than is ideal}
        \label{fig:mean and std of net44}
    \end{subfigure}
    \caption{Example of a dynamic minima in potential feild planning} 
    \label{fig:dynamicMinima}
\end{figure}

\subsection{Reachability Analysis}
\MC{Do we need to describe the basics of reachability analysis?}
